Decomposition of Decidable First-Order Logics over Integers and Reals

We tackle the issue of representing infinite sets of real- valued vectors. This paper introduces an operator for combining integer and real sets. Using this operator, we decompose three well-known logics extending Presburger with reals. Our decomposition splits a logic into two parts : one integer, and one decimal (i.e. on the interval [0,1]). We also give a basis for an implementation of our representation.

==> sec.extension.tex <==
\section{Extension of the known decidable logics}\label{sec:extension}

------------------------\\
Plan de la section :\\
- introduction de la logique PDM (attention si besoin dans section pr{\'e}c{\'e}dente)\\
\fbox{peut-{\^e}tre mettre le th{\'e}or{\`e}me \ref{thm:bounded} ici ?}\\
- PDM et RVA incomparables : RVA>PDM (puissances n{\'e}gatives), PDM>RVA(disque)\\
- prouver logique $\fo{\setD,+,*,\leq,W_b}$ d{\'e}cidable (RVA {\'e}tiquet{\'e} par polynomes et non pas codage binaire ?)\\
- proposer + la grande logique d{\'e}cidable connue : PDM+RVA (ie. $\fo{\setZ,+,\leq,V_b} \uplus \fo{\setD,+,*,\leq,W_b}$)\\
\fbox{piste : "puissances inverses $\cap$ irrationnels/disques"}\\
------------------------\\

\subsection{Presburger extended to Decimals with Multiplication (PDM)}
We study the expressivity of the decidable logic $\fo{\setZ,+,\leq}\uplus\fo{\setD,+,*,\leq}$ that naturally extends $\fo{\setR,\setZ,+,\leq}=\fo{\setZ,+,\leq}\uplus\fo{\setD,+,\leq}$.
%\begin{remark}
  %Note that the expressivity of $\fo{\setZ,+,\leq}\uplus\fo{\setD,+,*,\leq}$ is not comparable to the logic $\fo{\setZ,+,\leq,V_b}\uplus\fo{\setD,+,\leq,W_b}$ defining the class of sets representable by an RVA in basis $b$. Naturally, these two logics can be combined into $\fo{\setZ,+,\leq,V_b}\uplus\fo{\setD,+,*,\leq,W_b}$. Actually, the decidability of $\fo{\setD,+,*,\leq,W_b}$ is open.
%\end{remark}


\begin{center}
\setlength{\unitlength}{16pt}
\pssetlength{\psunit}{16pt}
\pssetlength{\psxunit}{16pt}
\pssetlength{\psyunit}{16pt}
\begin{tabular}[t]{c@{\hspace{.8cm}}c}
  \begin{picture}(5.5,5.5)(-1.25,-0.75)%
    %\put(-2.75,-1.75){\framebox(5.5,5.5){}}
    \psgrid[subgriddiv=1,gridcolor=black,griddots=5,gridlabels=7pt](0,0)(3,3)
    \pspolygon*[linecolor=black,fillcolor=black](0,0)(1,0)(0.5,1)
    \pspolygon*[linecolor=black,fillcolor=black](1,0)(2,0)(1.5,1)
    \pspolygon*[linecolor=black,fillcolor=black](1,1)(2,1)(1.5,2)
    \pspolygon*[linecolor=black,fillcolor=black](2,0)(3,0)(2.5,1)
    \pspolygon*[linecolor=black,fillcolor=black](2,1)(3,1)(2.5,2)
    \pspolygon*[linecolor=black,fillcolor=black](2,2)(3,2)(2.5,3)
    \rput(3.5,3.5){$\udots$}
    \rput(3.5,2.5){$\ldots$}
    \rput(3.5,1.5){$\ldots$}
    \rput(3.5,0.5){$\ldots$}
    %
    %%\psline[linecolor=black, linewidth=1pt](1,-1)(1,1)
    %%\psline[linecolor=blue,  linewidth=1pt](0,1)(0,2)
    %%\psline[linecolor=red,   linewidth=1pt](-1,2)(-1,3)
  \end{picture}
  &
  \begin{picture}(5.5,5.5)(-0.75,-0.75)%
    %\put(-2.75,-1.75){\framebox(5.5,5.5){}}
    \psgrid[subgriddiv=1,gridcolor=black,griddots=5,gridlabels=7pt](0,0)(3,3)
    \pscircle*[linecolor=black,fillcolor=black](0.5,0.5){0.5}
    \pscircle*[linecolor=black,fillcolor=black](1.5,0.5){0.5}
    \pscircle*[linecolor=black,fillcolor=black](1.5,1.5){0.5}
    \pscircle*[linecolor=black,fillcolor=black](2.5,0.5){0.5}
    \pscircle*[linecolor=black,fillcolor=black](2.5,1.5){0.5}
    \pscircle*[linecolor=black,fillcolor=black](2.5,2.5){0.5}
    \rput(3.5,3.5){$\udots$}
    \rput(3.5,2.5){$\ldots$}
    \rput(3.5,1.5){$\ldots$}
    \rput(3.5,0.5){$\ldots$}
    %
    %%\psline[linecolor=black, linewidth=1pt](1,-1)(1,1)
    %%\psline[linecolor=blue,  linewidth=1pt](0,1)(0,2)
    %%\psline[linecolor=red,   linewidth=1pt](-1,2)(-1,3)
  \end{picture}\\
  $\fo{\setR,\setZ,+,\leq}$
  &
  $\fo{\setZ,+,\leq}\uplus\fo{\setD,+,*,\leq}$ 
\end{tabular}
\end{center}


-------------

\begin{prp}
PDM and the logic underlying RVA are not comparable.
\end{prp}
\begin{proof}
Let two sets $E_1,E_2 \subseteq \partie{\setR^n}$ s.t. $E_1$ defined in $\fo{\setR,\setZ,+,\leq,V_r,W_r}$ and $E_2$ defined in $\fo{\setZ,+,\leq} \uplus \fo{[0,1[,+,\times,\leq}$. We show that $E_1$ is not PDM-definable and that $E_2$ is not RVA-representable.\\
Let us show that $E_1$ is not PDM-definable.\\ 
Let $E_1= \{ r^{-n} \mid r,n \in \setN\}$ (the negative powers of $r$). The following RVA represents $E_1$ (ie. its accepted language is $0 \star 0^*10^\omega$) : \fbox{dessiner le RVA !}
Assume $E_1$ PDM-definable ; then $E_1 = \cup_i D_i+Z_i$, where $i\in \setN$, $D_i\subseteq\partie{[0,1[^n}$, $Z_i\subseteq\partie{\setZ^n}$. Moreover $E_1 \in [0,1[$, hence $E_1=\cup_{i\mid 0\in Z_i}D_i$ : this means $E_1$ is definable in $\fo{[0,1[,+,\times,\leq}$. Thus, $E_1$ is of the form $\cup ( \cap P(x) \# c)$ where $\# \in \{ \leq,< \}$, $P(x)$ is a polynomial in $x$, and the union and intersection are finite. This means $E_1$ is a finite union of intervals, which contradicts the definition of $E_1$ being an infinite set of sparse points (the negative powers of $r$). Indeed, either each interval reduces to a single point, but there are infinitely many points and a finite number of intervals ; or there are two points in the same interval, but there are uncountably many points between those two, whereas the number of negative powers of $r$ is infinite but countable. Thus there exists an RVA-representable set which is not PDM-definable.\\
Let us show that $E_2$ is not RVA-representable.\\ 
Let $E_2 = \frac{\sqrt{2}}{2} = \{x\mid 2x^2=1\}$. The following PDM formula defines $E_2$ : $(x \times x)+(x \times x)=1$. Assume $E_2$ RVA-representable ; then this RVA is of the following form \fbox{dessiner le RVA !}. The sequence $\sigma$ leads to  an infinite path going through an accepting state. In the strongly connected component containing this infinite path, there is a path going from $\sigma$ to the accepting state, from which a word $\pi$ can be read infinitely often. Thus, the RVA accepts a word $\sigma \pi^\omega$, whose valuation is given by $\rho$. Then 
\begin{align*}
\rho (\sigma \pi^\omega) &= \rho(\sigma)+r^{-\vert\sigma\vert}.\rho(\pi)+r^{-(\vert\sigma\vert+\vert \pi\vert)}.\rho(\pi)+\ldots\\
&= \rho(\sigma)+\Sigma_{i=0}^\infty r^{-(\vert\sigma\vert+i.\vert \pi\vert)}.\rho(\pi) \\
&= \rho(\sigma)+r^{-\vert\sigma\vert}.\Biggl( \frac{1}{1-\frac{1}{r^{\vert \pi\vert}}} \Biggr).\rho(\pi)
\end{align*}
Hence $\rho (\sigma \pi^\omega) \in \setQ$ ; however $\sqrt{2} \notin \setQ$, thus there exists a PDM-definable set which is not RVA-representable.
\end{proof}

==> sec.knownclasses.tex <==
\section{Decomposition of Known Classes}\label{sec:knownclasses}

------------------------\\
Plan de la section :\\
- reguliers + RVA + NDD\\
- CPDBM\\
- poly{\`e}dres convexes, ...\\
------------------------\\

Known classes of sets are proved decomposable in this section.
 %%The expressiveness of $\fo{\setZ,+,\leq}\uplus\fo{\setD,+,*,\leq}$ is compared to other known logics in this section.


\subsection{Presburger logic extended to the reals}
In this section we prove that $\fo{\setR,\setZ,+,\leq}=\fo{\setZ,+,\leq}\uplus\fo{\setD,+,\leq}$. From this decomposition we deduce a geometrical characterization of the sets definable in this logic.

\medskip

First of all, observe that any set definable in the logic $\fo{\setZ,+,\leq}\uplus\fo{\setD,+,\leq}$ is also definable $\fo{\setR,\setZ,+,\leq}$. Conversely, the sets $\setR$ and $\setZ$, the function $+:\setR\times\setR\rightarrow\setR$ and the predicate $\leq$ are definable in $\fo{\setZ,+,\leq}\uplus\fo{\setD,+,\leq}$ from examples \ref{ex:set}, \ref{ex:eq}, \ref{ex:leq}, \ref{ex:sum}. Thus, stability by first order operations provides the following proposition :
\begin{prp}\label{prop:pres}
  $\fo{\setR,\setZ,+,\leq}=\fo{\setZ,+,\leq}\uplus\fo{\setD,+,\leq}$.
\end{prp}


Now, let us recall that sets definable in Presburger logic $\fo{\setZ,+,\leq}$ can be characterized thanks to \emph{linear sets} \cite{GS}. In fact, a set $Z\subseteq\setZ^n$ is definable in this logic if and only if it is equal to a finite union of linear sets $\vec{b}+P^*$ where $\vec{b}\in\setZ^n$, $P$ is a finite subset of $\subseteq \setZ^n$, and $P^*$ denotes the set of finite sums $\sum_{i=1}^k p_i$ with $p_1,\ldots,p_k\in P$ and $k\in\setN$. This geometrical characterization can be extended to the class of sets definable in $\fo{\setZ,+,\leq}\uplus\fo{\setD,+,\leq}$ by introducing the class of \emph{polyhedral convex sets}. A set $C\subseteq\setR^n$ is said \emph{polyhedral convex} if $C$ is defined by a finite conjunction of formulas $\scalar{\alpha}{\vec{x}}\#c$ where $\alpha\in\setZ^n$, $\#\in\{\leq,<\}$ and $c\in\setZ$. Recall that a \emph{Fourier-Motzkin quantification elimination} proves that a set $C\subseteq\setR^n$ is definable in $\fo{\setR,+,\leq}$ if and only if it is equal to a finite union of polyhedral convex sets. We have proved the following geometrical characterization :
\begin{thm} A set $R\subseteq \setR^n$ is definable in $\fo{\setR,\setZ,+,\leq}$ if and only if it is equal to a finite union of sets of the form $C+P^*$ where $C\subseteq\setR^n$ is a bounded polyhedral convex set and $P$ is a finite subset of $\setZ^n$.
\end{thm}

%%We now show that some known classes $\rondR\subseteq\partie{\setR^n}$ can be decomposed into $\rondR=\rondZ\uplus\rondD$ where $\rondZ\subseteq\partie{\setZ^n}$ and $\rondD\subseteq\partie{\setD^n}$. The classes we study here are Presburger definable sets \cite{FL08,Ler03,...}, Regular sets \cite{...Pythagore?}, and sets representable by DBM or CPDBM \cite{AD94?,...}.


\subsection{RVA}\label{sec:known:rva}
In this section, the class of sets representable by \emph{Real Vector Automata (RVA)} is proved decomposable.

\medskip

Let $b\geq 2$ be an integer called the \emph{basis of decomposition}. We denote by $\Sigma_b=\{0,\ldots,b-1\}$ the finite set of \emph{digits} and by $S_b=\{0,b-1\}$ the set of \emph{sign digits}. An infinite word $\sigma=\vec{s}\vec{a}_1\ldots\vec{a}_k\star\vec{a}_{k+1}\vec{a}_{k+2}\ldots$ over the alphabet $\Sigma_b^n\cup\{\star\}$ is said \emph{$b$-correct} if $\vec{s}\in S_b^n$ and $\vec{a}_i\in\Sigma_b^n$ for any $i\geq 1$. In this case, $\sigma$ is called a \emph{most significant digit first decomposition} of the following real vector $\rho_b(\sigma)\in \setR^n$:
  $$\rho_b(\sigma)=b^k\left(\frac{\vec{s}}{1-b}+\sum_{i\geq 1}b^{-i}\vec{a}_i\right)$$
A \emph{Real Vector Automaton (RVA)} in basis $b$ is a B{\"u}chi automaton $\automaton$ over the alphabet $\Sigma_b^n$ such that the language $\Lan{\automaton}$ recognized by $\automaton$ contains only $b$-correct words. The set $\inter{\automaton}$ represented by $\automaton$ is defined by $\inter{\automaton}=\{\rho_b(\sigma) \st \sigma\in\Lan{\automaton}\}$. A set $R\subseteq\setR^n$ is said \emph{$b$-recognizable} if there exists a RVA $\automaton$ in basis $b$ such that $R=\inter{\automaton}$. 

\medskip

According to \cite{Boigelot98}, the class of $b$-recognizable sets can be logically characterized by $\fo{\setR,\setZ,+,\leq,X_b}$ where $X_b$ is an additional predicate. The predicate $X_b$ over $\setR^3$ is such that $X_b(x,u,a)$ is true if and only if there exists a most significant digit first decomposition $\sigma=s a_1\ldots a_k\star a_{k+1}\ldots$ of $x$ and an integer $i\in\setN$ such that $a_i=a$ and $u=b^{k-i}$. 
\begin{thm}\cite{Boigelot98}
  A set $R\subseteq\setR^n$ is $b$-recognizable if and only if it is definable in $\fo{\setR,\setZ,+,\leq,X_b}$. 
\end{thm}

\medskip

In order to provide a decompostion of $\fo{\setR,\setZ,+,\leq,X_b}$, the predicate $X_b$ is proved expressible by two valuation functions $V_b$ and $W_b$ where :
\begin{itemize}
\item $V_b:\setZ\moins\{0\}\rightarrow\setZ$ is the \emph{integer valuation function} introduced in \cite{Bruyere94} and defined by $V_b(z)=b^j$, where $j\in\setZ$ is the greatest integer such that $b^{-j}z\in\setZ$.
\item $W_b:\setD\moins\{0\}\rightarrow \setD$ is the \emph{decimal valuation function} defined by $W_b(d)=b^j$, where $j\in\setZ$ is the least integer such that $b^{-j}d\not\in\setD$.
\end{itemize}
%%A set $R\subseteq\setR^n$ is said \emph{$r$-definable} if it can be defined in $\fo{\setR,\setZ,+,\leq,V_b,W_b}$. 

By expressing $X_b$ in $\fo{\setR,\setZ,+,\leq,V_b,W_b}$ and $V_b,W_b$ in $\fo{\setR,\setZ,+,\leq,X_b}$ we deduce that $\fo{\setR,\setZ,+,\leq,X_b}=\fo{\setR,\setZ,+,\leq,V_b,W_b}$. Finally, from proposition \ref{prop:pres} we get the following proposition.
\begin{prp}
  $\fo{\setR,\setZ,+,\leq, X_b}=\fo{\setZ,+,\leq, V_b}\uplus \fo{\setD,+,\leq, W_b}$.
\end{prp}
  %%  From \cite{Buyere94} we deduce that a set $R\subseteq\setR^n$ such that $\supp{f_R}$ is a finite class of subsets definable in $\textsf{FO}(\setZ,+,\leq,V_b)$ and such that $f_R(Z)$ is a $b$-regular set included in $\setD^n$ is $b$-regular. Conversely, let us consider a $b$-regular set $R\subseteq\setR^n$. Let $\automaton$ be a Buchi automaton that recognizes an $\omega$-regular language $\Lan{\automaton}$ of $b$-correct words and such that $R=\{\rho_b(\sigma) \st \sigma\in\Lan{\automaton}\}$. Let us denote by $t_1=(q_1\xrightarrow{\diamond}q_1'),\ldots,t_k=(q_k\xrightarrow{\diamond}q_k')$ the transitions of $\automaton$ labelled by $\diamond$. We denote by $\automaton_1,\ldots,\automaton_k$ the Buchi automata obtained from $\automaton$ by removing all the transitions labelled by $\diamond$ expect $t_i$. Naturally $\Lan{\automaton}\subseteq\Lan{\automaton_1}\cup\ldots\cup\Lan{\automaton_k}$. In fact, since $\automaton$ only accept words that contains exactly one occurrence of $\diamond$, we deduce the equality $\Lan{\automaton}=\Lan{\automaton_1}\cup\ldots\cup\Lan{\automaton_k}$. Thanks to the stability by finite union of $(\setR,\class)$ we can assume without loss of generality that $\automaton$ contains a unique transition labelled by $\diamond$. We denote this transition by $t_1=(q_1\xrightarrow{\diamond}q_1')$. Let us denote by $\automaton_Z$ the automaton obtained from $\automaton$ by removing the transition $t_1$ and by adding a fresh transition $q_1\xrightarrow{\diamond}q$ to a fresh accepting state $q$ and a fresh loop on $q$ labelled by $\{\vec{0}\}$. Let us also denote by $\automaton_D$ the automaton obtained from $\automaton$ by removing the transition $t_1$, by adding a fresh state $q_0'$ and a fresh transition $q_0'\xrightarrow{\diamond}q_1'$ and by replacing the initial state by $q_0'$. Note that $\automaton_Z$ and $\automaton_D$ recognize $\omega$-regular sets of $b$-correct words. Moreover the sets $Z=\{\rho_b(\sigma) \st \sigma\in\Lan{\automaton_Z}\}$ and $D=\{\rho_b(\sigma) \st \sigma\in\Lan{\automaton_D}\}$ satisfy $R=Z+D$, $Z\subseteq\setZ^n$ and $D\subseteq \left[0,1\right]^n$. From \cite{Bruyere94} we deduce that $Z$ is definable in $\textsf{FO}(\setZ,+,\leq,V_r)$. For any $J\subseteq\{1,\ldots,n\}$, let us denote by $D_I$ the set of $\vec{d}\in D$ such that $d_i=1$ if and only if $i\in I$ and $\unit_I\in\{0,1\}^n$ be the vector defined by $(\unit_I)_i=1$ if and only if $i\in I$. Observe that $R=\bigcup_{I}(\unit_I+Z)+(D_I-\unit_I)$ and $\unit_I+Z\subseteq\setZ^n$ is definable in $\textsf{FO}(\setZ,+,\leq,V_r)$ and $D_I-\unit_I\subseteq\setD^n$ is a $b$-regular set.


Moreover, it is clear that the logic $\fo{\setZ,+,\leq,V_b}\uplus\fo{\setD,+,\leq,W_b}$ extends $\fo{\setZ,+,\leq}\uplus\fo{\setD,+,\leq}$. However, even if the function $W_b$ is crucial to logically characterize the class of $b$-recognizable sets, this predicate is not used in practice. In fact, in order to get efficient algorithms for manipulating B{\"u}chi automata (more precisely, minimization and determinization), we only consider sets $R\subseteq\setR^n$ that can be represented by a \emph{weak RVA}. Recall that a B{\"u}chi automaton $\automaton$ is said \emph{weak} if any strongly connected component $S$ satisfies $S\subseteq F$ or $S\cap F=\emptyset$, where $F$ is the set of accepting states. Unfortunately, the class of sets $R\subseteq \setR^n$ representable by a weak RVA is not logically characterized since this class is not stable by first order operations (because of projection). In practice, since any set $R\subseteq\setR^n$ definable in $\fo{\setR,\setZ,+,\leq,V_b}$ can be represented by a weak RVA, the RVA symbolic representation is only used for representing sets in this logic. Just remark that $\fo{\setR,\setZ,+,\leq,V_b}=\fo{\setZ,+,\leq,V_b}\uplus \fo{\setD,+,\leq}$.



%%\TODO{Dire que $V_b$ a un interet limite. Que $W_b$ encore moins. Mais si on veux quand meme $V_b$ (avec des automates finis) on peut naturellement considerer $\fo{\setZ,+,\leq,V_b}\uplus\fo{\setD,+,*,\leq}$}


\subsection{CPDBM}
A DBM set $R$ is a set $R\subseteq\setR^n$ parameterized by a sequence $(c_{i,j})_{0\leq i,j\leq n}$ of elements in $\setZ\cup\{+\infty\}$ and a sequence $(\#_{i,j})_{0\leq i,j\leq n}$ of relations in $\{\leq,<\}$ such that we have the following equality (in which $r_0=0$) :
$$R=\{\vec{r}\in\setR^n \st \bigwedge_{0\leq i,j\leq n}r_i-r_j\#_{i,j}c_{i,j}\}$$
We denote by $\textrm{UDBM}$ the sequence $\textrm{UDBM}=(\textrm{UDBM}_n)_{n\in\setN}$ where $\textrm{UDBM}_n$ is the class of finite unions of DBM sets $R\subseteq \setD^n$.

\medskip

A CPDBM is a finite union of DBM sets where the parameters $(c_{i,j})_{1\leq i,j,\leq n}$ are constrained by a formula $\phi((c_{i,j})_{1\leq i,j,\leq n})$ in a logic $\fo{\setZ,\ldots}$ denoting either the decidable Presburger logic $\fo{\setZ,+,\leq}$ or the undecidable Peano logic $\fo{\setZ,+,*,\leq}$. More precisely, $\textrm{CPDBM}(\setZ,\ldots)$ denotes the class of finite unions of sets $R\subseteq\setR^n$ such that there exists a set $S\subseteq \setZ^{(n+1)^2}$ definable in $\fo{\setZ,\ldots}$ and a sequence $(\#_{i,j})_{0\leq i,j\leq n}$ of relations in $\{\leq,<\}$ such that:
$$R=\{\vec{r}\in\setR^n \st \exists (c_{i,j})_{0\leq i,j\leq n}\in S \ \bigwedge_{0\leq i,j\leq n}r_i-r_j\#_{i,j}c_{i,j}\}$$
%%We denote by $\textrm{UCPDBM}$ the sequence $\textrm{UCPDBM}=(\textrm{UCPDBM}_n)_{n\in\setN}$ where $\textrm{UCPDBM}_n$ is the class of finite union of CPDBM sets $R\subseteq\setR^n$.

\begin{prp}We have:
  \begin{itemize}
  \item $\textrm{CPDBM}(\setZ,+,*,\leq)=\fo{\setZ,+,*,\leq}\uplus \textrm{UDBM}$.
  \item $\textrm{CPDBM}(\setZ,+,\leq)=\fo{\setZ,+,\leq}\uplus \textrm{UDBM}$.
  \end{itemize}
\end{prp}
\begin{proof}
  The inclusion $\supseteq$ is immediate. For the converse, let $R\subseteq\setR^n$ be such that there exists a set $S\subseteq \setZ^{(n+1)^2}$ definable in $\textsf{FO}(\setZ,\ldots)$ and $(\#_{i,j})_{0\leq i,j\leq n}$ a sequence of relations in $\{\leq,<\}$ satisfying the previous equality. Let us consider the set $Z_{\vec{d}}=\setZ^n\cap (R-\vec{d})$ indexed by $\vec{d}\in\setD^n$. Observe that $Z_{\vec{d}}$ is the set of vectors $\vec{z}\in\setZ^n$ that satisfy the following equation, where $z_0=0=d_0$ :
  $$\exists (c_{i,j})_{0\leq i,j\leq n}\in S\ \bigwedge_{0\leq i,j\leq n}z_i-z_j\#_{i,j}c_{i,j}+(d_j-d_i)$$
  Note that $d_j-d_i\in\left]-1,1\right[$, and since $z_i-z_j,c_{i,j}\in\setZ$ we deduce that $z_i-z_j\#_{i,j}c_{i,j}+(d_j-d_i)$ is equivalent to $z_i-z_j\#_{i,j}c_{i,j}$ if $0\#_{i,j}d_j-d_i$, and it is equivalent to $z_i-z_j\#_{i,j}c_{i,j}-1$ otherwise. For any totally-defined function $h:\{0,\ldots,n\}^2\rightarrow\{0,1\}$, let us consider the set $D_h$ of vectors $\vec{d}\in\setD^n$ such that $0\#_{i,j}d_j-d_i$ iff $h(i,j)=0$ for any $0\leq i,j\leq n$. Note that $D_h$ is a DBM set included in $\setD^n$ and $Z_{\vec{d}}=I_h$ for any $\vec{d}\in D_h$ where:
  $$I_h=\{\vec{z}\in\setZ^n \st \exists (c_{i,j})_{0\leq i,j\leq n}\in S_k\ \bigwedge_{0\leq i,j\leq n}z_i-z_j\#_{i,j}c_{i,j}-h(i,j)\}$$
  From $R=\bigcup_{\vec{z}\in\setZ^n}\{\vec{z}\}+Z_{\vec{d}}=\bigcup_{h}\bigcup_{\vec{z}\in I_h}\{\vec{z}\}+D_h=\bigcup_{h}I_h+D_k$, we deduce that $R$ is definable in $\fo{\setZ,\ldots}\uplus \textrm{UDBM}$.
\end{proof}





%%\medskip

%%To establish the stability property, we introduce the class of semi-ID sets. An \emph{ID set} $S$ is a subset of $\setR^n$ of the form $S=I+D$ where $I\subseteq\setZ^n$ and $D\subseteq \setD^n$. A \emph{semi-ID set} is a finite union of ID sets. Observe that the interpretation of any finite IDF $f$ is a semi-ID set. We are going to prove that conversely the class of semi-ID sets and the class of finitely representable sets are equal.
%%\begin{remark}
%%  An ID set $S=I+D$ is finitely represented by the IDF $f$ satisfying $f(\emptyset)=\setD\moins D$, $f(I)=D$ and $f(J)=\emptyset$ for any $J\in\partie{\setZ^n}\moins\{\emptyset,I\}$.
%%\end{remark}









==> sec.preuves.tex <==

\section*{Technical Proofs}

\begin{anxDBM}We have %:
  %%\begin{itemize}
  %\item
$\bigcup\textrm{CP-DBM}_+=\fo{\setZ,+,\leq}\uplus \bigcup \textrm{DBM}_\setD$.
  %%\item $\textrm{CPDBM}(\setZ,+,\leq)=\fo{\setZ,+,\leq}\uplus \textrm{UDBM}$.
  %\end{itemize}
\end{anxDBM}
\begin{proof}
  Let us first prove the inclusion $\supseteq$. Let us consider a DBM $(\vec{c},\vec{\prec})$ denoting a set $D\subseteq\setD^n$ and a Presburger formula $\psi(\vec{x})$ denoting a set $Z\subseteq\setZ^n$ and let us prove that $Z+D$ is a $\bigcup\textrm{CP-DBM}_+$ set. Observe that $\vec{r}\in Z+D$ if and only if there exists $\vec{z}\in Z$ such that $\vec{r}-\vec{z}\in D$. The condition $\vec{r}-\vec{z}\in D$ is equivalent to $\bigwedge_{0\leq i,j\leq n}r_i-r_j\prec_{i,j} c_{i,j}+z_i-z_j$. Let us consider the Presburger formula $\psi(\vec{p}):=\exists \vec{z}\in\setZ^n\ p_{i,j}=c_{i,j}+z_i-z_j$ and observe that $R_{\psi,\vec{\prec}}=Z+D$. We have proved the inclusion $\supseteq$.

\smallskip

For the converse inclusion, let us consider a $\textrm{CP-DBM}_+$ set $R_{\vec{\phi},\vec{\prec}}$. Let $Z_{\vec{d}}=\setZ^n\cap (R_{\vec{\phi},\vec{\prec}}-\vec{d})$ indexed by $\vec{d}\in\setD^n$. Observe that $Z_{\vec{d}}$ is actually the following set of vectors :
  $$Z_{\vec{d}} = \bigcup_{\vec{c} \models \phi} \left\lbrace \vec{z} \in \setZ^n \vert \bigwedge_{0\leq i,j\leq n} z_i - z_j \prec_{i,j} c_{i,j} + (d_j - d_i) \right\rbrace$$
  Since $d_j-d_i\in\left]-1,1\right[$ and $z_i-z_j,c_{i,j}\in\setZ$ we deduce that $z_i-z_j\prec_{i,j}c_{i,j}+(d_j-d_i)$ is equivalent to $z_i-z_j\leq c_{i,j}$ if $d_i-d_j \prec_{i,j}0$ and it is equivalent to $z_i-z_j\leq c_{i,j}-1$ otherwise. Given a matrix $\vec{m}=(m_{i,j})_{0\leq i,j\leq n}$ such that $m_{i,j}\in\{0,1\}$ for any $0\leq i,j\leq n$, we denote by $I_{\vec{m}}$ and $D_{\vec{m}}$ the following sets:
 \begin{align*}
 I_{\vec{m}}&=\{ \vec{z}\in\setZ^n \mid \exists \vec{c}\ \phi(\vec{c})\wedge\hspace{-0.2cm}\bigwedge_{0\leq i,j\leq n}z_i-z_j\leq c_{i,j}-m_{i,j} \}\\
 D_{\vec{m}}&=\{\vec{d}\in\setD^n \mid \bigwedge_{0\leq i,j\leq n} (d_i-d_j\prec_{i,j}0 \Longleftrightarrow m_{i,j}=0)\}
\end{align*}
 Note that $D_{\vec{m}}$ is a DBM set and $Z_{\vec{d}}=I_{\vec{m}}$ for any $\vec{d}\in D_{\vec{m}}$. From $\bigcup_{\vec{m}}D_{\vec{m}}=\setD^n$ we deduce that $R_{\vec{\phi},\vec{\prec}}=\bigcup_{\vec{d}\in\setD^n}Z_{\vec{d}}+\{\vec{d}\}=\bigcup_{\vec{m}}I_{\vec{m}}+D_{\vec{m}}$. We have proved that $R_{\vec{\phi},\vec{\prec}}$ is definable in $\fo{\setZ,+,\leq} \uplus \bigcup\textrm{DBM}_\setD$.
\end{proof} 


\begin{anxUnion}
 % Let $f:\rondZ_n\longrightarrow\rondD_n$ be an IDF that represents a set $R$ and let $(I,D)\in\rondZ_n\times\rondD_n$. The set $R'=R\cup (I+D)$ is represented by the IDF $f':\rondZ_n\rightarrow\rondD_n$ defined by the following equality for any $Z'\subseteq\setZ^n$: $$f'(Z')=\Bigl(f(Z')\moins D\Bigr)\bigcup_{Z\st Z\cup I=Z'}\Bigl(f(Z)\cap D\Bigr)$$
Let $R \in \inter{IDF_{\rondZ_n \longrightarrow \rondD_n}}$. Then, for any $Z \in \partie{\setZ^n}$ and $D \in \partie{\setD^n}$, we also have $R \cup (Z+D) \in \inter{IDF_{\rondZ_n \rightarrow \rondD_n}}$.
\end{anxUnion}
\begin{proof}
  We consider an IDF $f:\rondZ_n \longrightarrow \rondD_n$ such that $\inter{f}=R$ and two sets $Z \in \partie{\setZ^n}$ and $D \in \partie{\setD^n}$. We must prove that there exists an IDF $f':\rondZ_n \longrightarrow \rondD_n$ such that $\inter{f'}=R'$ with $R'=R\cup (Z+D)$. We consider the following function:
  $$\begin{array}{cccl}
    f': 
    & \rondZ_n & \longrightarrow & \rondD_n\\
    &    Z'    & \longrightarrow & \displaystyle \Bigl(f(Z')\moins D\Bigr)\bigcup_{Z''\st Z''\cup Z=Z'}\Bigl(f(Z'')\cap D\Bigr)\\
  \end{array}$$
  As expected we are going to prove that $f'$ is an IDF such that $\inter{f'}=R'$. We first show that $f'$ is an IDF. First of all observe that $\bigcup_{Z'}f'(Z')=\setD^n$. Next, let $Z_1',Z_2'\in \rondZ_n$ such that $f'(Z_1')\cap f'(Z_2')\not=\emptyset$ then either $(f(Z_1')\moins D)\cap (f(Z_2')\moins D)\not=\emptyset$ or there exists $Z_1'',Z_2''$ such that $Z_1''\cup Z=Z_1'$ and $Z_2''\cup Z=Z_2'$ and $(f(Z_1'')\cap D)\cap(f(Z_2'')\cap D)\not=\emptyset$ since the other cases are not possible. But $(f(Z_1')\moins D)\cap (f(Z_2')\moins D)\not=\emptyset$ implies $f(Z_1')\cap f(Z_2')\not=\emptyset$ and since $f$ is an IDF we get $Z_1'=Z_2'$. And $(f(Z_1'')\cap D)\cap(f(Z_2'')\cap D)\not=\emptyset$ implies $Z_1''=Z_2''$ and in particular $Z_1'=Z_2'$. We have proved that $f'$ is an IDF. Finally, equality $\inter{f'}=R'$ comes from:
  \begin{align*}
    \inter{f'}
    =&\bigcup_{Z'}(Z'+f'(Z'))\\
    =&\bigcup_{Z'} \Bigl( (Z'+(f(Z')\moins D))\\
    &\bigcup_{Z'' \st Z''\cup Z=Z'}(Z'+(f(Z'')\cap D)) \Bigr) \\
    =&\bigcup_{Z'}(Z'+(f(Z')\moins D))\bigcup_{Z''}((Z''\cup Z)+(f(Z'')\cap D))\\
    =&\bigcup_{Z''}(Z''+((f(Z'')\moins D)\cup (f(Z'')\cap D)))\\
	&\cup (Z+D\cap (\bigcup_{Z''}f(Z'')))\\
    =&\inter{f}\cup (Z+D)
  \end{align*}
\end{proof}


\begin{anxUnique}
%$\inter{.}_{/IDF_{\rondZ \rightarrow \rondD}}$ is an injection.
For any $f_1,f_2 \in IDF_{\rondZ \rightarrow \rondD}$, $\inter{f_1}=\inter{f_2} \implies f_1=f_2$ .
\end{anxUnique}
\begin{proof}
  Consider $Z_1\subseteq \setZ^n$ and let $\vec{d}\in f_1(Z_1)$. As $(f_2(Z))_{Z}$ forms a sharing of $\setD^n$, there exists $Z_2$ such that $\vec{d}\in f_2(Z_2)$. Let $\vec{z}_1\in Z_1$ and observe that $\vec{r}_1=\vec{z}_1+\vec{d}\in \inter{f_1}$ and from $\inter{f_1}=\inter{f_2}$ we get $\vec{r}_1\in \inter{f_2}$. Thus, there exists $Z_2'$ such that $\vec{r}_1\in Z_2'+f_2(Z_2')$. Since $Z_2'\subseteq \setZ^n$ and $f_2(Z_2')\subseteq \setD^n$ we get $\vec{z}_1\in Z_2'$ and $\vec{d}\in f_2(Z_2')$. As $(f_2(Z))_{Z}$ forms a sharing of $\setD^n$ and $\vec{d}\in f_2(Z_2)\cap f_2(Z_2')$ we get $Z_2=Z_2'$. In particular $\vec{z}_1\in Z_2$ and we have proved that $Z_1\subseteq Z_2$. Next, let us consider $\vec{z}_2\in Z_2$. From $\vec{r}_2=\vec{z}_2+\vec{d}\in\inter{f_2}$ and $\inter{f_2}=\inter{f_1}$ we deduce that $\vec{r}_2\in \inter{f_1}$ and once again we deduce that there exists $Z_1'$ such that $\vec{r}_2\in Z_1'+f_1(Z_1')$. As $(f_1(Z))_{Z}$ forms a sharing of $\setD^n$, as previously we deduce that $Z_1'=Z_1$ and we get $\vec{z}_2\in Z_1$. We have proved that $Z_1=Z_2$. Therefore, $f_1(Z_1)\subseteq f_2(Z_1)$ for any $Z_1$. By symmetry we deduce that $f_1(Z)=f_2(Z)$ for any $Z$ and we have proved that $f_1=f_2$.
\end{proof}

